Sketching and Sequence Alignment: A Rate-Distortion Perspective

Pairwise alignment of DNA sequencing data is a ubiquitous task in bioinformatics and typically represents a heavy computational burden. A standard approach to speed up this task is to compute "sketches" of the DNA reads (typically via hashing-based techniques) that allow the efficient computation of pairwise alignment scores. We propose a rate-distortion framework to study the problem of computing sketches that achieve the optimal tradeoff between sketch size and alignment estimation distortion. We consider the simple setting of i.i.d. error-free sources of length $n$ and introduce a new sketching algorithm called "locational hashing." While standard approaches in the literature based on min-hashes require $B = (1/D) \cdot O\left( \log n \right)$ bits to achieve a distortion $D$, our proposed approach only requires $B = \log^2(1/D) \cdot O(1)$ bits. This can lead to significant computational savings in pairwise alignment estimation.

==> intro_old.tex <==


A key step in many bioinformatics analysis pipelines is the identification of regions of
similarity between pairs of sequences (typically DNA sequencing reads).
This task, known as (pairwise) sequence
alignment, is a heavy computational burden,
particularly in the context of sequencing data from long-read sequencing technologies such as PacBio and Oxford Nanopore.
% , which produce noisy reads.
% The advent of long-read sequencers such as PacBio and Oxford Nanopore have
% enabled us to obtain reads that are thousands of base pairs long, making 
% made the goal of obtaining gold-standard genome assemblies a reality.
%  Unlike short read 
% technologies, which provide reads of length $100$-$200$ bp with an error rate of 
% $1\%$ chiefly consisting of substitution errors, 
These technologies typically produce DNA reads of lengths in the tens of thousands,
but at the expense of significantly higher error rates ($\sim\hspace{-1mm} 10\%$)
% with a nominal error rate of $13$-$15\%$, consisting mostly of insertions and deletions
\cite{pacbio_errorRate}.
% While the long reads make resolving repeated sequences easier,








% This issue is commonly addressed via a two-step approach: first, we filter pairs
% of reads which are likely to have a large alignment,
% % and then do more computationally intensive 
% % processing on such pairs.
% and then we perform computationally intensive alignment algorithms only on the selected pairs.
% The \emph{Jaccard similarity} between the set of $k$-mers of each read can be 
% shown to be a proxy for the alignment size, and is usually used as the filter.
% % A full dynamic-programming-based alignment is then performed only on pairs of reads with high Jaccard similarity.
% This strategy has the added benefit that the Jaccard similarities don't need to be computed exactly, and can instead be efficiently estimated through the use of \emph{min-hashes}.
% This is done by hashing all $k$-mers of a read and computing the minimum hash value (the min-hash) for each read. 
% For a randomly chosen hash function, the probability that the min-hashes are the same for two distinct reads is precisely their $k$-mer Jaccard similarity (JS). 
% Hence, 
% % given a set of random hash functions, 
% one can estimate the Jaccard similarity by computing the fraction of min-hash collisions out of the set of hash functions considered.






% Assembly of long noisy read data is usually performed based on the  \emph{overlap-layout-consensus} (OLC) paradigm \cite{olc}, illustrated in Figure~\ref{fig:olc}(a).
% % \noindent \emph{\bf Algorithmic challenges.} %in the assembly of long reads: }
% % Traditional assembly algorithms based on \emph{de Bruijn} graphs
% % are usually too sensitive to the high error rates of long-read sequencing technologies.
% % In practice, assembly of long reads is accomplished by a three-step procedure, known as \emph{overlap-layout-consensus} (OLC).
% % In the overlapping step,
% First, 
% pairwise read alignment \cite{pairwise} is used to identify \emph{approximate} overlaps between pairs of reads. 
% Then, in the layout step, an 
% \emph{assembly graph} is constructed. 
% Each read is a node and a (weighted) directed edge $(u,v)$ implies that the suffix of $u$ approximately matches the prefix of $v$.
% % ``significant'' overlap. 
% % Ideally, 
% % at the end of this procedure 
% The true genome then corresponds to a path that visits every node on the assembly graph, or a \emph{Hamiltonian} path. 
% % By finding a Hamiltonian cycle 
% % For the sake of parsimony, the path corresponding to the shortest sequence is preferred.
% % As such, the assembly problem becomes NP-hard under most OLC-based formulations, and 
% % heurisitcs are used to extract the final sequence from the graph.
% Finally, in the consensus step, 
% % we exploit 
% the 
% redundancy in the overlaps between consecutive reads in the Hamiltonian path is exploited to correct errors.


% Genome assembly is usually performed based on one of two main approaches:  
% \emph{de-novo} assembly, where one attempts to assemble a new genome ``from scratch'' using only the reads obtained, and \emph{reference-based}
% assembly, where one assembles the reads using a pre-assembled genome of a
% related organism. 
% Alignment is an integral part of most
% pipelines in either approach, and is often the most time consuming step (see Fig. \ref{fig:assembly_times}). % and \cite[Figure S11]{Kamath2017}).
% In both settings naive dynamic programming  
% based alignment \cite{NeedlemanWunch, SmithWaterman, myers1986ano} 
% is impractical due to its quadratic time complexity.

% In reference-based 
% assembly pipelines \cite{vaser2017fast, Wick2019}, 
% where one has a
% reference of a related organism, the first 
% step usually consists of aligning all reads
% to the reference;
% % -- colloquially read-to-reference alignment. % IS: not very colloquial to me
% i.e., read-to-reference alignment.
% %Naively, this step entails computing sequence alignments
% %with the reference
% %for reads, a dynamic programming problem with cost the product 
% %of the read length and reference length.
% For $n$ reads each of length $L$ and a reference of length $G$,
% the time complexity of aligning all reads to the reference via
% dynamic programming is $O(nLG)$, which is impractical 
% in settings where there are $n \sim 10^5$ reads, each of length 
% $L \sim 10^4$, with $G$ on the order of $10^6$-$10^{11}$
% depending on the organism. 


% Most genome assembly pipelines for noisy long-read sequencing data \cite{HGAP, Berlin2015, li2016minimap, Chin2016, Koren2017, Kamath2017, Shasta} are based on the overlap-layout-consensus paradigm, described in Figure~\ref{fig:olc}(a) (although alternative approaches have been proposed \cite{ABruijn,Flye}).
% The first step in this paradigm -- overlapping -- 
% essentially corresponds to computing the size of the largest prefix-suffix match between each pair of reads, as illustrated in Figure~\ref{fig:alignment}(a).
% % This step is also referred to as \emph{pairwise alignment}, a
% % More generally, 
% The term \emph{alignment} refers more generally to finding any matches (not just prefix-suffix) between two sequences, 
% % both overlaps and internal matches, 
% but for simplicity we will treat the words overlap and alignment as interchangeable. 
% While fast methods exist for finding \emph{exact} overlaps \cite{sga,bwa}, 
% when the reads are noisy, finding approximate overlaps is a heavy computational burden and consumes most of the assembly computation time, as shown in Figure~\ref{fig:alignment}(b).
% Naively, this step entails computing sequence alignments
% for all pairs of reads, a dynamic programming problem with cost quadratic in the read length \cite{NeedlemanWunch, SmithWaterman, myers1986ano}. 
% For $n$ reads each of length $\ell$, the time complexity of aligning all pairs of reads 
% would be $O(n^2\ell^2)$. 
% Even for bacterial genome datasets where
% the number of reads obtained is on the order of $n \sim 10^5$, with 
% $\ell \sim 10^4$, this is impractical.


The optimal alignment between two strings of length $\ell$ can be found via dynamic programming in $O(\ell^2)$ time \cite{SmithWaterman}.
Hence, the time complexity for the pairwise alignment of $n$ reads of length $\ell$ is $O(n^2 \ell^2)$, which is impractical even for bacterial genome datasets (for which we may have $n \sim 10^5$ and long reads with $\ell \sim 10^4$).
This challenge is commonly addressed 
by first converting each long DNA sequence into a short \emph{sketch} of length $h$. The sequence sketch be thought of as low-dimensional representation of the read, and is typically constructed using hashing techniques.
The sketching procedure is designed in such a way that estimating the alignment score between two sequences from their corresponding sketches is straightforward and can essentially be performed in $O(h)$ time.
Most practical sequence alignment pipelines perform pairwise hashing comparisons first (in $O(n^2h)$ time), and then perform more careful alignment only on a small set of selected pairs that are ``likely'' to have a significant alignment
% using hashing-based approaches to efficiently \emph{estimate} pairwise alignments and select pairs that are likely to have large overlaps
\cite{Myers2014,Berlin2015,li2016minimap,li2018minimap2}.
% Since in practical settings  most pairs have no overlap \cite{HINGE}, one is  left with relatively few pairs of reads, for which precise alignments can be computed.




% \iscomment{say that we use overlap and alignment interchangeably. just say alignment everywhere?}


% % Then, computationally intensive alignment algorithms are applied only to the selected pairs.
% % This approach can greatly speed up pairwise alignment/overlapping because, in practical sequencing datasets, most pairs of reads have no overlap \cite{HINGE}.


% % , one  only cares about the
% % alignment between reads with a large sequence identity or overlap.

% % % via a two-step approach: first, 




% an alignment estimation procedure is used to 
% % the pairs
% % of reads are filtered so that those 
% identify those
% pairs that are likely to have a large alignment. % are identified.
% % and then do more computationally intensive 
% % processing on such pairs.
% Then, computationally intensive alignment algorithms are applied only to the selected pairs.
% This two-step approach can greatly speed up the alignment task because, in practice, one  only cares about the
% alignment between reads with a large sequence identity or overlap.
% % Further, as shown in Figure \ref{fig:ovlp_hist}, in a typical dataset, more than $99.99\%$ of 
% % pairs of reads do not have a significant 
% % overlap.
% % Hence, efficiently identifying such pairs of reads can lead to significant savings.






This approach can be cast under the more general framework of sketching algorithms \cite{indyk2007sketching}, which are becoming increasingly popular in genomic data science \cite{sketching_review,marcais_sketching}.


For each read, one constructs a low-dimensional representation, or sketch, typically using hash functions.
The sketches are designed so as to facilitate the estimation of pairwise alignments.
As a concrete example, we consider the MHAP algorithm \cite{Berlin2015}, illustrated in Figure~\ref{fig:alignment}(c).
% Several works have
% % exploited this idea and 
% developed ways to efficiently
% estimate pairwise alignments
% % identify pairs of reads with large overlaps
% \cite{Myers2014,Berlin2015,li2016minimap,li2018minimap2}.
% The proposed algorithms typically rely on hashing to efficiently find pairs of reads that share many $k$-mers (length-$k$ contiguous substrings).
% Particularly relevant to our discussion is the MHAP algorithm of \cite{Berlin2015}.
% The basic idea of the MHAP algorithm is as follows.
Suppose we want to estimate the overlap size between two reads $r_0$ and $r_1$ and let $\Gamma(r_i)$ be the set of all $k$-mers (length-$k$ contiguous substrings) in $r_i$. %, $i=0,1$.
For a hash function $h : \Sigma^k \to \Z$, where $\Sigma = \{\bA,\bC,\bG,\bT\}$, we define the \emph{min-hash} of a read $r_i$, with slight abuse of notation, to be
\al{
    h(r_i) :=
    \min \{h(x) :  x \in \Gamma(r_i)\}.
}
% for each read $r_i$.
A min-hash sketch of size $m$ for read $r_i$ can then be defined as 
$[h_1(r_i),h_2(r_i),...,h_m(r_i)]$ 
% $[h_1(\Gamma(r_i)),...,h_m(\Gamma(r_i))]$ 
based on $m$ distinct hash functions $h_1,...,h_m$.
The key motivation behind this sketching scheme, originally proposed in \cite{broder1997syntactic_minHash}, is that
% The key observation behind MHAP is that, 
for a randomly selected hash function $h$ (so that all $k$-mers are equally likely to be the minimizer of $h$),
\begin{align}
    % \Pr\left[ h(\Gamma(r_0)) =  h(\Gamma(r_1))\right] =
        \Pr\left[ h(r_0) =  h(r_1)\right] =
    \frac{|\Gamma(r_0) \cap \Gamma(r_1)|}{|\Gamma(r_0) \cup \Gamma(r_1)|}.
    \label{eq:prjk}
\end{align}
The right-hand side of (\ref{eq:prjk}) is known as the \emph{Jaccard similarity} between the sets of $k$-mers $\Gamma(r_0)$ and $\Gamma(r_1)$, which we denote by $\js_k(r_0,r_1)$.
The observation in (\ref{eq:prjk}) implies that
% In other words, 
the binary indicator function $\one\{h(r_0) = h(r_1)\}$ is an unbiased estimator for $\js_k(r_0,r_1)$.
% the Jaccard similarity between $\Gamma(r_0)$ and $\Gamma(r_1)$.
% between the sets $\Gamma(r_0)$ and $\Gamma(r_1)$.
Under the assumption that the reads are error-free and that $r_0$ and $r_1$ do not share many $k$-mers outside of the overlap, $\js_k(r_0,r_1)$ is approximately equal to the overlap fraction (or, more generally, to the total alignment fraction).
% (Figure~\ref{fig:alignment}(a)).
% The observation in Eq.~(\ref{eq:prjk}) \cite[Section 3.3.3]{mmds} implies that 
As illustrated in Figure~\ref{fig:alignment}(c), given sketches $S_0$ and $S_1$, one can thus estimate the overlap fraction $\theta$ between $r_0$ and $r_1$ by computing the fraction of coordinates where $S_0$ and $S_1$ have the same value or, equivalently, computing
\al{
\hat \theta = \frac1m \sum\nolimits_{j=1}^m \one\{h_j(r_0) = h_j(r_i)\}.
% \nolimits
\label{eq:mhap}
}
This procedure is known to be robust to read errors, as the $k$-mer Jaccard similarity remains proportional to the overlap fraction in expectation under fairly general noise models \cite{MHAP,sjs_cell}.



\begin{figure}[b!] %[h] %[b!]
\vspace{-5mm}
\centering
%\hspace{-5mm}
\includegraphics[width = 0.99\columnwidth]{figs/alignment_fig6.pdf}
%\hspace{-5mm}
%\subfigure[\label{fig:timebreakdown}]{\includegraphics[width = .3\columnwidth]{figs/timebreakdown.pdf}}
\vspace{-1mm}
    \caption{(a) The overlap fraction between two reads can be defined as the size of the largest prefix-suffix match divided by the length spanned by  the two reads when aligned. 
    When reads have errors, determining the overlap fraction is more challenging.
    (b) Breakdown of the compute time for the HINGE assembly pipeline \cite{HINGE} on three bacterial genome datasets; 
    (c) Estimating the overlap fraction between two reads using min-hash-based sketches \cite{Berlin2015}.
    % Computing the overlap fraction for noisy reads 
    \label{fig:alignment}}
% \vspace{-5mm}
\end{figure}

==> problem02-02.tex <==
% !TEX root = main.tex


The general distributed source coding problem \cite{slepianwolf,AhlswedeKorner,WynerSide,WynerZiv} 
is concerned with the compression of correlated sources by encoders that do not communicate with each other.
In our setting, instead of being correlated, the two length-$n$ source sequences $X_1$ and $X_2$ have an overlap of size $\theta n$. 
% , for some $\theta \in (0,1)$.
We assume that the unknown overlap parameter satisfies $\theta \in \{0\} \cup [\theta_0,1]$ for some fixed  $\theta_0 > 0$.
This is because typically in practice one is not interested in accurately estimating small overlaps, only no-overlaps or moderately sized overlaps \cite{kamath2020adaptive}.


Our goal is to design an encoder (i.e., a sketching procedure) with small encoding rates and a decoder that takes the sketches and attempts to estimate the (normalized) overlap size $\theta$.
% outputs an overlap estimate $\hat \theta$ with a small expected distortion $E[d(\theta,\hat\theta)]$ for some distortion metric $d$.
We focus on a quadratic distortion metric, thus requiring
the decoder to produce an estimator $\hat \theta$ 
satisfying (\ref{eq:dist}).
% that satisfying
% \al{
% E[(\theta - \hat \theta)^2] \leq D. \label{eq:dist}
% }


For a sequence length $n$, the joint distribution $(X_1,X_2)$ is defined as follows.
% \iscomment{should we make $\theta$ fixed?}
% First, an overlap parameter $\theta$ is drawn at random from $(0,1)$ according to a pdf $f(\theta)$ to be specified.
First, a single i.i.d.~$\Ber(1/2)$ sequence $X$ of length $(2-\theta)n$ is generated.
In the context of DNA sequencing, $X$ can be thought of as the underlying genome sequence.
We then define $X_1 = X[1:n]$ (the first $n$ bits of $X$) and $X_2 = X[(1-\theta)n + 1: (2-\theta)n]$ (the last $n$ bits of $X$).
Notice that the length-$\theta n$ suffix of $X_1$ matches the length-$\theta n$ prefix of $X_2$.
In this paper, we assume that $X_1$ and $X_2$ are not corrupted by noise.
Extensions to the more realistic noisy setting are briefly discussed in Section~\ref{sec:discussion}.

We will also define the \emph{overlap fraction} $\alpha$ to be the ratio between the overlap size $\theta n$ and the length of $X$; i.e.,
% better parameterization for this problem is to consider the  parameter
\al{
\alpha \triangleq \frac{\theta n}{(2-\theta)n} = \frac{\theta}{2-\theta}. 
}
Notice that $\alpha \in (0,1)$ and $\theta$ are in one-to-one correspondence.
As it turns out, parameterizing the problem in terms of $\alpha \in (0,1)$ is more natural.
Hence, 
% we will assume that the goal of the decoder is to produce an estimator $\hat \alpha$ (instead of $\hat \theta$) that satisfies a quadratic distortion constraint
% \al{
% E[(\alpha - \hat \alpha)^2] \leq D. \label{eq:dist}
% }
% Moreover, 
\iscomment{remove this?}
we will assume that $\alpha$ is drawn uniformly at random from $(0,1)$, and let $f(\theta)$ be the distribution induced on $\theta$ via $\theta = \alpha/(1+\alpha)$.


% The first $n$ bits of this sequence yield $X_1$, while the last 

% To model two sources $X_1$ and $X_2$ with an overlap fraction $\theta$, we use a single underlying stochastic source $X$ (the ``genome'' source) that generates a sequence of length
% % $(2-\theta)n$, 
% $2n/(1+\theta)$
% which is split into three segments: one of length  
% % $(1-\theta)n$ 
% $n(1-\theta)/(1+\theta)$
% that is only part of $X_1$, one of length 
% % $\theta n$ 
% $n(2\theta)/(1+\theta)$
% that is part of both $X_1$ and $X_2$ and one of length  
% % $(1-\theta)n$ 
% $n(1-\theta)/(1+\theta)$
% that is only part of $X_2$.
% Each source may be independently corrupted by noise.









% At a high level, the goal of sketch-based pairwise alignment is to compress reads into a typically sublinear-size sketch from which pairwise alignments can be accurately estimated.
% In general, sketches do not need to be $k$-mer min-hashes, and it is not clear 
% whether testing the presence of fixed-length $k$-mers is the optimal sketching scheme for a given noise model.
% This suggests that a \emph{source coding} framework could be useful in characterizing 
% the informational 







Unlike in standard source coding, where a length-$n$ source $X_i$ is compressed into $n R$ bits, for a positive rate $R$, the regime of interest for our problem requires sketches of constant size in $n$.
Our main results show that this is in fact feasible.

% \iscomment{move this para to problem setting?}
% Notice that a priori it is unclear whether $B$ needs to scale with $n$ in order for the problem to be feasible.
% In standard rate-distortion theory, the number of bits $B(n)$ used to compress a length-$n$ source is linear in $n$, and we are interested in the \emph{rate} $R = B(n)/n$ that is achievable for a given distortion constraint.


% with a given positive rate $R_i$ leading to a linear-size representation, we are interested in compressing length-$n$ source sequences to a size that is sublinear in $n$.
% Figure~\ref{fig:sourcecoding} illustrates one possible such encoding, namely a histogram of the frequency of several strings of different lengths.
% Notice that the total size of this type of histogram representation 
% % (including the counts) 
% is logarithmic in $n$
% % This suggests 
% % the following notion of sketching rate.
% suggesting that we should 
% % that, for this problem, we should 
% modify the standard definition of encoding rate 
% % in source coding problems 
% as follows.
% % Instead, we will say that 


\begin{defn}
A sketching procedure with sketch length $B$ is a mapping 
% An encoder is said to produce length-$B$ sketches if 
$\Sk : \{0,1\}^n \to \{0,1\}^B$.
% $\Enc_i : \{0,1\}^n \to \{1,...,2^{R_i\log n }\}$
% with sketching rate $R_i$ is a mapping .
\end{defn} 



The sketching procedure is independently applied to each source, producing $\hat X_i = \Sk(X_i)$.
The decoder's task is then to estimate $\theta$ from 
$\hat X_1$ and $\hat X_2$.

\begin{defn}
A decoder is any function $\Dec : \{0,1\}^B \times \{0,1\}^B \to (0,1)$.
\end{defn}

The decoder is used to estimate $\hat \theta = \Dec(\hat X_1,\hat X_2)$.
We say that a rate-distortion pair $(B,D)$ is achievable if, for sufficiently large $n_0$, there exists a sketching procedure for any $n \geq n_0$ with sketch length $B$ satisfying (\ref{eq:dist}).
Naturally, the rate-distortion function is defined as $B(D) = \inf \{B : (B,D) \text{ is achievable}\}$.


\vspace{2mm}
\noindent {\bf Notation: }
Throughout we assume that $\log(\cdot)$ refers to the base-$2$ logarithm.
For $x \in \R$, we let $(x)^+ = \max(x,0)$.
For a positive integer $m$ we let $[1:m] = \{1,\dots,m\}$.
For a real number $x \in (0,1)$, we let  
% \gkcomment{address non-uniqueness} 
$x = \sum_{i=1}^\infty x_i 2^{-i}$, $x_i \in \{0,1\}$, be its (minimal) binary expansion and for some $b \in \Z_+$, we let 
\aln{
[x]_b \triangleq \sum_{i=1}^b x_i 2^{-i}
} 
be a $b$-bit truncation of $x$.






==> problem05-09.tex <==
% !TEX root = main.tex

The general distributed source coding problem \cite{slepianwolf,AhlswedeKorner,WynerSide,WynerZiv} 
is concerned with the compression of correlated sources by encoders that do not communicate with each other.
In our setting, instead of being correlated, the two length-$n$ source sequences $X_1$ and $X_2$ have an overlap of size $\theta n$. 
% , for some $\theta \in (0,1)$.
We assume that the unknown overlap parameter satisfies $\theta \in \{0\} \cup [\theta_0,1]$ for some fixed  $\theta_0 > 0$.
This is because typically in practice one is not interested in accurately estimating small overlaps, only no-overlaps or moderately sized overlaps \cite{kamath2020adaptive}.


Our goal is to design an encoder (i.e., a sketching procedure) with small encoding rates and a decoder that takes the sketches and attempts to estimate the (normalized) overlap size $\theta$.
% outputs an overlap estimate $\hat \theta$ with a small expected distortion $E[d(\theta,\hat\theta)]$ for some distortion metric $d$.
We focus on a quadratic distortion metric, thus 
seeking a decoder
that produces an estimator $\hat \theta$ 
satisfying (\ref{eq:dist}) for some $D$.
% that satisfying
% \al{
% E[(\theta - \hat \theta)^2] \leq D. \label{eq:dist}
% }


For a sequence length $n$, the joint distribution $(X_1,X_2)$ is defined as follows.
% \iscomment{should we make $\theta$ fixed?}
% First, an overlap parameter $\theta$ is drawn at random from $(0,1)$ according to a pdf $f(\theta)$ to be specified.
First, a single i.i.d.~$\Ber(1/2)$ sequence $X$ of length $(2-\theta)n$ is generated.
In the context of DNA sequencing, $X$ can be thought of as the underlying genome sequence.
We then define $X_1 = X[1:n]$ (the first $n$ bits of $X$) and $X_2 = X[(1-\theta)n + 1: (2-\theta)n]$ (the last $n$ bits of $X$).
Notice that the length-$\theta n$ suffix of $X_1$ matches the length-$\theta n$ prefix of $X_2$.
In this paper, we assume that $X_1$ and $X_2$ are not corrupted by noise.
Extensions to the more realistic noisy setting are briefly discussed in Section~\ref{sec:discussion}.

We will also define the \emph{overlap fraction} $\alpha$ to be the ratio between the overlap size $\theta n$ and the length of $X$; i.e.,
% better parameterization for this problem is to consider the  parameter
\al{
\alpha \triangleq \frac{\theta n}{(2-\theta)n} = \frac{\theta}{2-\theta}. 
\label{eq:alpha}
}
Notice that $\alpha \in (0,1)$ and $\theta$ are in one-to-one correspondence.
% As it turns out, parameterizing the problem in terms of $\alpha \in (0,1)$ is more natural.
% Hence, 
% we will assume that the goal of the decoder is to produce an estimator $\hat \alpha$ (instead of $\hat \theta$) that satisfies a quadratic distortion constraint
% \al{
% E[(\alpha - \hat \alpha)^2] \leq D. \label{eq:dist}
% }
% Moreover, 
% \iscomment{remove this?}
% we will assume that $\alpha$ is drawn uniformly at random from $(0,1)$, and let $f(\theta)$ be the distribution induced on $\theta$ via $\theta = \alpha/(1+\alpha)$.


% The first $n$ bits of this sequence yield $X_1$, while the last 

% To model two sources $X_1$ and $X_2$ with an overlap fraction $\theta$, we use a single underlying stochastic source $X$ (the ``genome'' source) that generates a sequence of length
% % $(2-\theta)n$, 
% $2n/(1+\theta)$
% which is split into three segments: one of length  
% % $(1-\theta)n$ 
% $n(1-\theta)/(1+\theta)$
% that is only part of $X_1$, one of length 
% % $\theta n$ 
% $n(2\theta)/(1+\theta)$
% that is part of both $X_1$ and $X_2$ and one of length  
% % $(1-\theta)n$ 
% $n(1-\theta)/(1+\theta)$
% that is only part of $X_2$.
% Each source may be independently corrupted by noise.









% At a high level, the goal of sketch-based pairwise alignment is to compress reads into a typically sublinear-size sketch from which pairwise alignments can be accurately estimated.
% In general, sketches do not need to be $k$-mer min-hashes, and it is not clear 
% whether testing the presence of fixed-length $k$-mers is the optimal sketching scheme for a given noise model.
% This suggests that a \emph{source coding} framework could be useful in characterizing 
% the informational 







Unlike in standard source coding, where a length-$n$ source $X_i$ is compressed into $n R$ bits, for a positive rate $R$, the regime of interest for our problem requires sketches of constant size in $n$.
Our main results show that this is in fact feasible.

% \iscomment{move this para to problem setting?}
% Notice that a priori it is unclear whether $B$ needs to scale with $n$ in order for the problem to be feasible.
% In standard rate-distortion theory, the number of bits $B(n)$ used to compress a length-$n$ source is linear in $n$, and we are interested in the \emph{rate} $R = B(n)/n$ that is achievable for a given distortion constraint.


% with a given positive rate $R_i$ leading to a linear-size representation, we are interested in compressing length-$n$ source sequences to a size that is sublinear in $n$.
% Figure~\ref{fig:sourcecoding} illustrates one possible such encoding, namely a histogram of the frequency of several strings of different lengths.
% Notice that the total size of this type of histogram representation 
% % (including the counts) 
% is logarithmic in $n$
% % This suggests 
% % the following notion of sketching rate.
% suggesting that we should 
% % that, for this problem, we should 
% modify the standard definition of encoding rate 
% % in source coding problems 
% as follows.
% % Instead, we will say that 


\begin{defn}
A sketching procedure with sketch length $B$ is a mapping 
% An encoder is said to produce length-$B$ sketches if 
$\Sk : \{0,1\}^n \to \{0,1\}^B$.
% $\Enc_i : \{0,1\}^n \to \{1,...,2^{R_i\log n }\}$
% with sketching rate $R_i$ is a mapping .
\end{defn} 



The sketching procedure is independently applied to each source, producing $\hat X_i = \Sk(X_i)$.
The decoder's task is then to estimate $\theta$ from 
$\hat X_1$ and $\hat X_2$.

\begin{defn}
A decoder is any function $\Dec : \{0,1\}^B \times \{0,1\}^B \to (0,1)$.
\end{defn}

The decoder is used to estimate $\hat \theta = \Dec(\hat X_1,\hat X_2)$.
We say that a rate-distortion pair $(B,D)$ is achievable if, for sufficiently large $n_0$, there exists a sketching procedure for any $n \geq n_0$ with sketch length $B$ satisfying 
% (\ref{eq:dist}).
\al{
\max_{\theta} E[(\theta - \hat \theta)^2] \leq D.
\label{eq:maxdist}
}
The rate-distortion function $B(D)$ (i.e., the minimum number of sketching bits needed to guarantee distortion $D$) is defined as $B(D) = \inf \{B : (B,D) \text{ is achievable}\}$.



\vspace{2mm}
\noindent {\bf Notation: }
Throughout we assume that $\log(\cdot)$ refers to the base-$2$ logarithm.
For $x \in \R$, we let $(x)^+ = \max(x,0)$.
For a positive integer $m$ we let $[1:m] = \{1,\dots,m\}$.
For a real number $x \in (0,1)$, we let  
% \gkcomment{address non-uniqueness} 
$x = \sum_{i=1}^\infty x_i 2^{-i}$, $x_i \in \{0,1\}$, be its (minimal) binary expansion and for some $b \in \Z_+$, we let 
\aln{
[x]_b \triangleq \sum_{i=1}^b x_i 2^{-i}
} 
be a $b$-bit truncation of $x$.






==> proof02-23.tex <==
% !TEX root = main.tex

% In this section, we provide the additional details required to complete the proof of Theorem~\ref{thm:main}.




% In order to analyze the scheme, we first describe more formally the construction of the estimator $\hat \alpha$ from Section~\ref{sec:multipleloc}.
% \begin{itemize}
%     \item need to say that we ignore zero values
% \end{itemize}


In this section we provide the key steps to prove the achievability of Theorem~\ref{thm:main}.
\ifarxiv
Proofs of lemmas and the proof of the converse result are relegated to the Appendix.
\else
Proofs of lemmas and the proof of the converse result are relegated to a longer version of this manuscript \cite{sketchinglong}.
\fi

The key step in the analysis of our sketching procedure and its decoder is obtaining, for the $j$th lexicographic ordering, $j \in [1:u]$, bounds for the pmf
\aln{
p_j(k) \triangleq \Pr \left( [m_{1,j}/n]_v - [m_{2,j}/n]_v = k \, 2^{-v} \right). 
}
Intuitively, this pmf has a probability mass of $\alpha$  near $k \approx (1-\theta)2^v$, and no other probability mass anywhere.
% More precisely, we establish the following lemma.
This is made precise in the following lemma.
\begin{lemma} \label{lem:pmf}
If 
$\K = \{ k : \  |k \, 2^{-v} - (1-\theta)| \leq 2^{-(v-1)}\}$, 
then
% For any $j \in [1:u]$, 
% \aln{
% \Pr \left( (1-\beta) - 2^{-(v-1)} \leq [m_{1,j}/n]_v - [m_{2,j}/n]_v \leq (1-\beta) + 2^{-(v-1)} \right). 
% }
\al{
\sum_{k \in \K} p_j(k) \geq \alpha - \ep_n,
\label{eq:lemeq1}
}
where $\lim_{n\to \infty} \ep_n = 0$.
Moreover,
\al{
\max \{ p_j(k) : k \notin \K \} \leq 
2^{-(v-1)}. \label{eq:lemeq2}
% \frac{1}{\b2^}.
}
\end{lemma}
Given the lemma, we can bound the expected distortion as follows.
First, we note that the set $\K$ from Lemma~\ref{lem:pmf} has cardinality at most $5$ (as we work with a resolution of $2^{-v}$ and are considering
an interval of length $4 \times 2^{-v}$).
Hence, for $n$ large enough, there is at least one value of $k \in \K$ with $p_j(k) \geq \alpha/6$.
%
% Notice that, while the random variables $[ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v$, $1 \leq j \leq u$, are not technically independent, as $n \to \infty$, they are essentially independent.
% This is because, given the location $m_{i,j}$ of the lexicographically first suffix based on one 
Notice that, 
since the $u$ different lexicographic orderings are chosen independently at random,
% if we view each of the $u$ masks $Z$ as drawn independently and uniformly at random from $\{0,1\}^n$, 
$(m_{1,j},m_{2,j})$ is independent of $(m_{1,\ell},m_{2,\ell})$ for $j \ne \ell$.
Hence, the random variables $[ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v$, for $1 \leq j \leq u$, are independent (and identically distributed).

We bound the distortion by considering two separate cases.
If $\alpha = 0$ (which is equivalent to $\theta = 0$), then the estimator will be $\hat \theta = 0$ as long as no element of $\A$ appears more than $\alpha_0 u / 6$ times, and the distortion will be zero.
If this condition is violated for some element $k2^{-v}$ with $k \in \K$, then we incur a distortion of at most $(2^{-(v-1)})^2$.
If this condition is violated for some $k2^{-v}$ with $k \notin \K$, then the distortion can be at most $1$, but this happens with low probability, as shown in the following lemma (which holds regardless of whether $\alpha = 0$).
\begin{lemma} \label{lem:bins}
The probability that there is a value $k2^{-v}$ for $k \notin \K$ that appears more than $\alpha_0 u/12$ times in $\A$ is at most
\al{
\exp \left[ -2 u ( \alpha_0/12 - u 2^{-(v-1)})^2 \right],
\label{eq:alpha0u}
}
provided that $\alpha_0/12 > u 2^{-(v-1)}$.
\end{lemma}
% Notice that there are at most $u$ distinct values in $\A$.
% Using the union bound, Hoeffding's inequality, and (\ref{eq:lemeq2}),  the probability that there is a value $k2^{-v}$ for $k \notin \K$ that appears more than $\alpha_0 u/12$ times in $\A$ is at most
% \al{
% u \exp \left[ -2 u ( \alpha_0/12 - 2^{-(v-1)})^2 \right],
% \label{eq:alpha0u}
% }
% % for any $\delta > 0$,
% as long as $\alpha_0/12 > 2^{-(v-1)}$.
% \iscomment{set $\alpha_0$}.
Hence, when $\alpha = 0$ the expected distortion satisfies
\al{
E & [(\theta-\hat \theta)^2 ]  
 \leq 2^{-2(v-1)} + e^{-2u(\frac{\alpha_0}{12} - u 2^{-(v-1)} )^2}.
% \\
% &  \leq 25 \cdot 2^{-(v-1)} + (u+1) e^{-2u(\alpha/24)^2}. 
\label{eq:multipleloc1}
}
Next we consider the case $\alpha \geq \alpha_0$.
Notice that in this case Lemma~\ref{lem:bins} still holds.
Moreover, the probability that, for no $k \in \K$, $k2^{-v}$ appears at least $(\alpha_0/12)u$ times in $\A$ is at most
\al{
\exp \left( -2 u (\alpha/6-\alpha_0/12)^2 \right) \leq \exp \left( -2 u (\alpha_0/12)^2 \right).
}
We conclude that, if
$\alpha_0/12 > u2^{-(v-1)}$, 
% the probability that the resulting estimator is $\hat \theta = k \, 2^{-v}$ for some $k \notin \K$ is at most 
% \al{
% (u+1) \exp \left[ -2 u ( \alpha_0/12 - 2^{-(v-1)})^2 \right].
% }
% We conclude that 
the expected distortion in the case $\alpha \geq \alpha_0$ can bounded as 
% Hence, in the case $\alpha = 0$, the expected distortion can be bounded as
\al{
E [(\theta-\hat \theta)^2 ]  
 & \leq 2^{-2(v-1)} + e^{-2u(\frac{\alpha_0}{12} - u2^{-(v-1)} )^2} + e^{-2u(\frac{\alpha_0}{12})^2} \nonumber \\
 & 
  \leq 2^{-2(v-1)} + 2 e^{-2u(\frac{\alpha_0}{12} - u 2^{-(v-1)} )^2}.
\label{eq:multipleloc2}
}
Since the right-hand side of (\ref{eq:multipleloc2}) is greater than the right-hand side of (\ref{eq:multipleloc1}), we can take (\ref{eq:multipleloc2}) to be a bound for both cases.

Finally, by setting $v = \alpha_0 \sqrt{B} /24$ $u = B/v$, we obtain 
% (after some algebra)
% \iscomment{check}
\al{
E & [(\theta-\hat \theta)^2 ] 
% \leq ( 24 \sqrt{B} /\alpha_0 + 2) \exp\left(-\sqrt{B} \alpha_0 / 24 \right),
\leq 3 \exp\left(-\sqrt{B} \alpha_0 / 24 \right),
}
which holds for $B$ large enough.
% as long as $v > \log(24/\alpha_0)$.
This implies that 
% the rate-distortion function satisfies
$
% \ln\left( \frac{1}{D} \right) \geq \frac{\alpha_0 \sqrt{B}}{24} - \ln\left( \frac{24 \sqrt{B}}{\alpha_0} + 2 \right),
\ln\left( 3/D \right) \geq \alpha_0 \sqrt{B}/24,
% \; \Rightarrow \; 
% - \ln\left( 3 \right),
$
which yields the bound in Theorem~\ref{thm:main}.
Since this bound only holds for $B$ large enough, 
% (since we require $u2^{-(v-1)} < \alpha_0/12$), 
our bound on $B(D)$ only holds for small enough $D$.

% Now we analyze the resulting distortion by considering two separate cases, depending on the value of $\alpha$.
% If $\alpha > 6 \alpha_0$, then the probability that, for no $k \in \K$, $k2^{-v}$ appears at least $\alpha_0 u$ times is at most
% \aln{
% \exp \left( -2 u (\alpha/5 - \alpha_0)^2 \right)
% \leq \exp \left( -2 u (\alpha_0/5)^2 \right).
% }
% Notice that, as long as $\alpha_0 - 2^{-(v-1)} > \alpha_0/5
% \Leftrightarrow \alpha_0 > \tfrac54 2^{-(v-1)}$, 
% % \Rightarrow \alpha_0 > 2^{-(v-1)}$, 
% % By setting $\delta = \alpha/12$, we conclude that, if 
% % $\alpha/12 > 2^{-(v-1)}$, 
% the probability that the resulting estimator is $\hat \theta = k \, 2^{-v}$ for some $k \notin \K$ is at most 
% \al{
% (u+1) \exp \left[ -2 u ( \alpha_0/5)^2 \right].
% }
% Therefore, when $\alpha > 6 \alpha_0$, the distortion satisfies
% \al{
% E & [(\theta-\hat \theta)^2| \alpha ]  \nonumber \\
% & \leq \alpha 2^{-2(v-1)} 
% + (1-\alpha) (u+1) e^{-2u(\alpha_0/5)^2}.
% % \nonumber \\
% % &  \leq 2^{-2(v-1)} + (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)} )^2},
% % \\
% % &  \leq 25 \cdot 2^{-(v-1)} + (u+1) e^{-2u(\alpha/24)^2}. 
% \label{eq:multipleloc2-case1}
% }
% Now we consider the second case, when $\alpha < 6 \alpha_0$.
% In this case, $\theta = \frac{2\alpha}{1+\alpha} < 12 \alpha_0$.
% Notice that, if there is no value $k2^{-v}$ for $k \notin \K$ that appears more than $\alpha_0 u$ times in $\A$, then we either have $\hat \theta = 0$ or $\hat \theta = k 2^{-v}$ for some $k \in \K$.
% Using (\ref{eq:alpha0u} again, we conclude that, when $\alpha < 6 \alpha_0$, 
% the distortion satisfies
% \al{
% E & [(\theta-\hat \theta)^2| \alpha ]  
% % \nonumber \\
% % & 
% \leq 
% \max( (12\alpha_0)^2, 2^{-2(v-1)} )
% + u e^{-2u(\alpha_0/5)^2}.
% % & \leq \alpha 2^{-2(v-1)} 
% % + (1-\alpha) (u+1) e^{-2u(\alpha_0/5)^2}.
% \label{eq:multipleloc2-case2}
% }
% If we set $\alpha_0 = \tfrac{1}{12} 2^{-(v-1)}$,
% we obtain a general bound 
% \al{
% E & [(\theta-\hat \theta)^2| \alpha ]  \nonumber \\
% & \leq 2^{-2(v-1)} 
% + (u+1) e^{-2u(2^{-(v-1)}/60)^2}.
% \label{eq:multipleloc2-combined}
% }
% Moreover, the probability that, for no $k \in \K$, $k2^{-v}$ appears at least $(\alpha/6-\delta)u$ times is at most
% $\exp \left( -2 u \delta ^2 \right)$.




% it still holds that the probability that there is a value  is at most (\ref{eq:alpha0u}).
% Hence, 



% If $\alpha \leq \alpha_0{\bf /2}$, then the probability that the estimator outputs some






% % Thus, we can use Hoeffding's inequality to establish that 



% % Notice that there are at most $u$ values in $\A$.
% % Using the union bound, Hoeffding's inequality, and (\ref{eq:lemeq2}),  the probability that there is a value $k2^{-v}$ for $k \notin \K$ that appears more than $(\alpha/6 - \delta)u$ times in $\A$ is at most
% % \al{
% % u \exp \left[ -2 u ( \alpha/6 - \delta - 2^{-(v-1)})^2 \right],
% % }
% % for any $\delta > 0$,
% % as long as $\alpha/6 - \delta > 2^{-(v-1)}$.
% % IS: Moving this up:
% % Moreover, the probability that, for no $k \in \K$, $k2^{-v}$ appears at least $(\alpha/6-\delta)u$ times is at most
% % $\exp \left( -2 u \delta ^2 \right)$.
% By setting $\delta = \alpha/12$, we conclude that, if 
% $\alpha/12 > 2^{-(v-1)}$, the probability that the resulting estimator is $\hat \theta = k \, 2^{-v}$ for some $k \notin \K$ is at most 
% \al{
% (u+1) \exp \left[ -2 u ( \alpha/12 - 2^{-(v-1)})^2 \right].
% }
% We conclude that the expected distortion can bounded as 
% \al{
% E & [(\theta-\hat \theta)^2| \alpha ]  \nonumber \\
% & \leq \alpha 2^{-2(v-1)} 
% + (1-\alpha) (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)} )^2} \nonumber \\
% &  \leq 2^{-2(v-1)} + (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)} )^2},
% % \\
% % &  \leq 25 \cdot 2^{-(v-1)} + (u+1) e^{-2u(\alpha/24)^2}. 
% \label{eq:multipleloc2}
% }
% as long as $\alpha/12 \leq 2^{-(v-1)}$.
% Since $\alpha$ is uniformly distributed in $(0,1)$,
% $\Pr(\alpha/24 \leq 2^{-(v-1)}) = 24 \cdot 2^{-(v-1)}$, and by averaging (\ref{eq:multipleloc2}) over $\alpha$, we obtain
% \aln{
% E [(\theta-\hat \theta)^2 ] &  \leq  24 \cdot 2^{-(v-1)} + 2^{-2(v-1)}  \nonumber \\
% & \quad  + (u+1) E_\alpha \left[ e^{-2u(\alpha/12 - \alpha/24 )^2} \right] \\
% &  \leq 25 \cdot 2^{-(v-1)} + (u+1) E_\alpha \left[ e^{-2u(\alpha/24)^2}\right] \\
% & = 25 \cdot 2^{-(v-1)} + (u+1) \frac{\sqrt{\pi} (1-2Q(\sqrt{u} /12))}{2\sqrt{2 u}  /24}
% % \label{eq:multipleloc2}
% }
% % \iscomment{It looks like this doesn't decay exponentially in $u$?}
% % \iscomment{To get exponential decay, we need to assume that $\alpha$ is bounded away from zero. It makes sense since for $\alpha$ close to zero, the estimator is not good}


% % \iscomment{what is a good way to bound that integral?}








==> proposal.tex <==

At a high level, the goal of sketch-based pairwise alignment is to compress reads into a typically sublinear-size sketch from which pairwise alignments can be accurately estimated.
In general, sketches do not need to be $k$-mer min-hashes, and it is not clear 
whether testing the presence of fixed-length $k$-mers is the optimal sketching scheme for a given noise model.
This suggests that a \emph{source coding} framework could be useful in characterizing 
the informational 

\begin{figure}[h] %[h] %[b!]
% \vspace{-1mm}
\centering
% \hspace{-3mm}
\includegraphics[width = .9\columnwidth]{figs/sourcecoding3.pdf}
% \vspace{-4mm}
    \caption{A distributed lossy source coding framework for sketching-based sequence alignment.
    \label{fig:sourcecoding}}
% \vspace{-3mm}
\end{figure}
limits of this problem.
In particular, a distributed (lossy) source coding framework \cite{Aaron2Terminal} seems fitting.
The general distributed source coding problem \cite{slepianwolf,AhlswedeKorner,WynerSide,WynerZiv} 
is concerned with the compression of correlated sources by encoders that do not communicate with each other.
For our setting, shown in Figure~\ref{fig:sourcecoding}, the two sources correspond to two reads and the ``correlation'' is their overlap fraction $\theta$.
Unlike in standard source coding, where encoder $\Enc_i$ compresses source $X_i$ with a given positive rate $R_i$ leading to a linear-size representation, we are interested in compressing length-$n$ source sequences to a size that is sublinear in $n$.
Figure~\ref{fig:sourcecoding} illustrates one possible such encoding, namely a histogram of the frequency of several strings of different lengths.
Notice that the total size of this type of histogram representation 
% (including the counts) 
is logarithmic in $n$
% This suggests 
% the following notion of sketching rate.
suggesting that we should 
% that, for this problem, we should 
modify the standard definition of encoding rate 
% in source coding problems 
as follows.
% Instead, we will say that 


\begin{defn}
An encoder $\Enc_i$ with sketching rate $R_i$ is a mapping $\Enc_i : \Sigma^n \to \{1,...,2^{R_i\log n }\}$.
\end{defn} 


The goal is to design encoders with low sketching rates and a decoder that takes the sketches and outputs an overlap estimate $\hat \theta$ with a small expected distortion $E[d(\theta,\hat\theta)]$ for some distortion metric $d$.
To model two sources $X_1$ and $X_2$ with an overlap fraction $\theta$, we use a single underlying stochastic source $X$ (the ``genome'' source) that generates a sequence of length
% $(2-\theta)n$, 
$2n/(1+\theta)$
which is split into three segments: one of length  
% $(1-\theta)n$ 
$n(1-\theta)/(1+\theta)$
that is only part of $X_1^n$, one of length 
% $\theta n$ 
$n(2\theta)/(1+\theta)$
that is part of both $X_1^n$ and $X_2^n$ and one of length  
% $(1-\theta)n$ 
$n(1-\theta)/(1+\theta)$
that is only part of $X_2^n$.
Each source may be independently corrupted by noise.



A natural first step is to consider the error-free case and let the underlying source $X$ be an i.i.d.~sequence with symbols chosen uniformly from $\Sigma = \{0,1\}$.
Consider the min-hash sketching scheme described in Figure~\ref{fig:alignment}(c) with $k$-mer length $k = 2\log n$ and $m$ hash functions.
It is straightforward to show that 
the non-overlapping parts of $X_1$ and $X_2$ do not share any identical segment of length $2\log n$ with probability tending to $1$.
Hence, a min-hash collision $h(X_1) = h(X_2)$ happens if and only if the minimizing $k$-mer is in the overlap, which happens with probability $\theta$.
This means that (\ref{eq:mhap}) is the maximum likelihood estimator for $\theta$ and it is distributed as $\tfrac{1}{m}\cdot{\rm Binomial}(m,\theta)$.
Under the quadratic metric $d(\theta,\hat\theta) = (\theta-\hat\theta)^2$, the achieved distortion is simply the variance of the estimator, which is $\theta(1-\theta)/m$.
Notice that the size of the sketch is $2 m \log n$ bits, since we need to specify $m$ minimizing $k$-mers, for $k = 2 \log n$, and the sketching rate of the encoders is $2m$.
We conclude that, in this i.i.d.~error-free
setting, sketching rate $2m$ can provide overlap estimates with expected distortion $\theta(1-\theta)/m$, upper-bounding the rate-distortion function as $R(D) \leq 2 \lceil \theta(1-\theta)/D \rceil$.



This simple example paves the way for several research questions.
Even for i.i.d.~noise-free sources, it is unclear whether the standard min-hash sketching above (i.e., rate-distortion pair $(2m,\theta(1-\theta)/m)$) is optimal.
Moreover, when $X_1$ and $X_2$ are independently corrupted by noise (say through a binary symmetric channel), 
the scenario is more complicated.
Because of the noise, length-$k$ substrings in the overlap 
% may be likely to 
may be corrupted in one of the sources, reducing the  probability of a desired min-hash collision.
On the other hand, hashing shorter strings increases the chances of spurious collisions, and a sweet spot must be found.
Furthermore, when the sources are non-uniform and non-i.i.d.~(e.g., Markov sources are known to capture certain compositional features of bacterial genomes \cite{greenberg2019metagenomic}), different substrings of the same length may have different probabilities.
In this case, ideas from variable-length source coding such as Huffman or Lempel-Ziv coding \cite{cover2012elements} may be useful towards the characterization of variable-length optimal sketching.


Developing a general rate-distortion theory for sketching 
genomic sequence data will have applications beyond pairwise alignment, since sketching is becoming a ubiquitous task in genomic data science to reduce storage requirements \cite{sketching_review} and to allow sublinear complexity algorithms \cite{marcais_sketching}.

==> result02-02.tex <==
% !TEX root = main.tex



Our main contribution is a new sketching procedure that significantly improves over the required number of bits $B$ 
% to achieve a distortion $D$ 
in (\ref{eq:mhapbits}).
Combined with a simple lower bound on the minimum sketch size, we have the following main result.

\begin{theorem} \label{thm:main}
The minimum sketch size $B$ required to achieve achieve distortion $D$  satisfies
\al{
\tfrac18 \log (1/D) \leq B(D) 
\leq {\color{blue} \bf C} \log^2 (1/D).
}
\end{theorem}


We first introduce the new sketching technique and then analyze its performance.


\subsection{Locational Hashing} \label{sec:simpleloc}

Our sketching procedure is motivated by the min-hash approach from Section~\ref{sec:minhash}.
But instead of recording the minimizer $k$-mers of certain hash functions, we record the approximate \emph{location} of special substrings in the sequence $X_i$.


We start by introducing a simple construction that stores only one locational hash, and then improve upon it.
Suppose we have a sequence $X_1$ for which we want to compute a sketch $\hat X_1$.
We start by lexicographically sorting the set 
\aln{
\S = \{X_1 [m:n]\cdot \$ : 1 \leq m \leq n\}
}
of all suffixes of $X_1$.
To make the sorting operation well-defined, we append to each suffix $X_1 [m:n]$ a character $\$$, which is assumed to be the last character in the lexicographic order of the alphabet.
We then take the lexicographically first string from $\S$, and its corresponding location $m_1$.
Notice that, for the case of binary strings, this {\color{blue} essentially} corresponds to taking the starting point of the longest run of zeros in $X_1$
\gkcomment{not exactly true. Will have ties with constant probability} (but the lexicographic approach extends to larger alphabets). 


Our sketch will be constructed by storing the first $B$ bits of the binary expansion of $m_1/n$; i.e.,
% \aln{
% \Sk(X_1) = \left( \lfloor 2^1 m/n \rfloor, \lfloor 2^2 m/n \rfloor, \dots, \lfloor 2^B m/n \rfloor \right).
% }
% \aln{
% % \Sk(X_1) 
% \hat X_1
% = 2^{-B} \lfloor 2^B m_1/n \rfloor.
% }
\aln{
% \Sk(X_1) 
\hat X_1
= [ m_1/n ]_B.
}
% Notice that storing $\hat X_1$ requires exactly $B$ bits.
% Also 
Notice that the difference between $[ m_1/n ]_B$ and $m_1/n$ is at most $2^{-B}$.
Let $m_2$ and $\hat X_2$ be the counterparts of $m_1$ and $\hat X_1$ for $X_2$.
The decoder can then estimate the overlap $\theta$ from the sketches $\hat X_1$ and $\hat X_2$ by simply setting
% \al{
% \hat \alpha = (\hat X_1 - \hat X_2)^+.
% }
\al{
\hat \theta = 1- (\hat X_1 - \hat X_2)^+.
}
To analyze the performance of this estimator, consider the original length-$(2-\theta)n$ sequence $X$, from which $X_1$ and $X_2$ were generated.
Notice that, for large $n$, the location of the lexicographically first suffix of $X$ is essentially uniformly distributed over all possible starting locations.
Hence the probability that the lexicographically first suffix of $X$ falls in the overlap between $X_1$ and $X_2$ approaches
\aln{
\frac{\theta n}{(2-\theta)n} = \alpha
}
as $n \to \infty$.
This implies that, with probability approaching $\alpha$, the lexicographically first suffix of $X_1$ and $X_2$ corresponds to the same location in $X$, and we have
\al{
m_1 = m_2 + (1-\theta) n.
\label{eq:shift}
}
Thus, with a probability approaching $\alpha$, the estimator satisfies
\aln{
|\theta - \hat \theta| \leq  2\cdot 2^{-B} = 2^{-(B-1)}.
}
Whenever (\ref{eq:shift}) is not satisfied (which occurs with probability approaching $1-\alpha$ as $n \to \infty$), the absolute error of the estimator is at most $1$, which implies that
\al{
E[(\theta-\hat \theta)^2 ] \leq \alpha 2^{-2(B-1)} + (1-\alpha). \label{eq:simpleloc}
}
% \iscomment{no averaging?}
% By averaging over $\alpha$, we obtain a distortion bound $2^{-2B} + 1/2$. 
% \iscomment{not $1/2$?}
We see that the locational hashing approach to sketching allows us to obtain a term in the distortion bound (\ref{eq:simpleloc}) of the form $2^{-B}$.
However, because the estimator only ``works'' with probability $\alpha$, our achieved distortion cannot go below $1-\alpha$.
In the next subsection, we fix this issue by repeating the locational hashing procedure for distinct lexicographic orders.




\subsection{Improved Locational Hashing} \label{sec:multipleloc}


In order to improve on the performance of the sketching procedure in Section~\ref{sec:simpleloc}, we consider using different lexicographic orders to compare strings (while maintaining \$ as the last 
character in the lexicographical order).
We do this by picking an ordering of $0$ and $1$ at each 
position uniformly at random, independent across positions. 
In other words for position $i$ of the suffix, $1 > 0 > \$$ 
with probability 0.5 and $0>1>\$$ with probability $0.5$.

Using the lexicographical orderings thus generated, we
order our suffixes obtained from $X_1$ and $X_2$. 
We note that with any lexicographic ordering so generated, 
we still have a collision from overlap of $X_1$
and $X_2$ with probability approaching $\alpha$ as $n\to \infty$.
 
% One way to define a new lexicographic ordering is by defining a random ``mask'' sequence $Z$ chosen uniformly at random from $\{0,1\}^n$ {\color{red}(inspired by Shannon ciphers)}.
% Then, for two binary sequences $a$ and $b$, each of length at most $n$, we can compare $a$ and $b$ by first xor-ing each of them with $Z$, and then comparing the resulting sequences lexicographically.

In order to build the improved sketch, we consider two parameters, $u$ and $v$.
We then generate $u$ different lexicographic orderings to compute $u$ different starting locations $m_{i,1},\dots,m_{i,u}$ for the lexicographically first suffix of $X_i$.
We build our sketch of $X_i$ by taking the $v$-bit truncation of $m_{i,j}/n$, for $j=1,\dots,u$; i.e.,
\al{
% \Sk(X_i) = \left( 
% 2^{-v} \lfloor 2^v m_{i,1}/n \rfloor, \dots,
% 2^{-v} \lfloor 2^v m_{i,u}/n \rfloor
% \right).
\Sk(X_i) = \left( 
[ m_{i,1}/n ]_v, \dots,
[ m_{i,u}/n ]_v 
\right).
}
Notice that this sketch requires $B=uv$ bits.
For 
% of the $u$ lexicographic orderings, 
$j \in [1:u]$,
\aln{
% 1-(2^{-v} \lfloor 2^v m_{1,j}/n\rfloor - 2^{-v} \lfloor 2^v m_{2,j}/n \rfloor )^+
1-([ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v )^+
}
% $(1-m_{1,j}-m_{2,j})^+$ 
is an estimator for $\theta$ with the same performance as (\ref{eq:simpleloc}).
Moreover, in expectation, $\alpha u$ of them will satisfy
\al{
& m_{1,j} - m_{2,j} = (1-\theta) n 
% \nonumber \\
% \Rightarrow \; &
% 2^{-v} \lfloor 2^v m_{1,j}/n \rfloor - 2^{-v} \lfloor 2^v m_{2,j}/n\rfloor = (1-\theta) + \delta_j,
\label{eq:shift2}
}
and thus 
\al{
% 2^{-v} \lfloor 2^v m_{1,j}/n \rfloor - 2^{-v} \lfloor 2^v m_{2,j}/n\rfloor = (1-\theta) + \delta_j,
[ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v = (1-\theta) + \delta_j,
\label{eq:errorperentry}
}
where $\delta_j$ is an error term due to the finite-bit representation, and satisfies $|\delta_j| \leq 2\cdot 2^{-v}$.

Notice that, intuitively, for the remaining $(1-\alpha)u$ indices $j$, the value of $(m_{1,j}-m_{2,j})/n$ will be distributed in $(0,1)$ and is not expected to concentrate on any particular value.
Hence, an intuitive estimator for $\theta$ is obtained by 
% setting $\hat \theta = 1-a$, where $a$ 
letting $a$ be
the most frequent value (i.e., the mode) in the set
\aln{
\A = \{ [ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v : 1 \leq j \leq u \},
}
and then setting $\hat \theta = 1-a$ if $a\geq 0$ and $\hat \theta = 0$ if $a < 0$.
% If that value is negative, we set $\hat \theta = 0$.
% the largest set of indices $j \in [1:u]$ such that the corresponding values of (\ref{eq:errorperentry}) are all within $2 \cdot 2^{-v}$ of each other, and outputting any of those values as $\hat \theta$.
We make one final modification to this estimator.
If the mode of $\A$ appears less than $\alpha_0 u$ times (for some $\alpha_0$ to be determined), then we simply output $\hat \theta = 0$.


In the next subsection, 
% we describe how this argument can be made formal, and
we show that the resulting distortion satisfies
\iscomment{need to update}
\al{
E & [(\theta-\hat \theta)^2| \alpha ] \nonumber
\\ &  \leq\alpha 2^{-2(v-1)} 
 + (1-\alpha) (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)})^2}. \label{eq:multipleloc}
}
It is easy to see that the expected distortion achieved with sketches of length $B = uv$ is significantly better than what is achieved with a single locational hash (\ref{eq:simpleloc}) and with the min-hash-based approach (\ref{eq:mhapbits}).
Moreover, by setting $u = ${\bf ??} and $v = ${\bf ??}, we obtain the upper bound in Theorem~\ref{thm:main}.




\subsection{Analysis}


% In order to analyze the scheme, we first describe more formally the construction of the estimator $\hat \alpha$ from Section~\ref{sec:multipleloc}.
% \begin{itemize}
%     \item need to say that we ignore zero values
% \end{itemize}



The key step in the analysis of our sketching procedure and its decoder is obtaining, for the $j$th lexicographic ordering, $j \in [1:u]$, bounds for the pmf
\aln{
p_j(k) \triangleq \Pr \left( [m_{1,j}/n]_v - [m_{2,j}/n]_v = k \, 2^{-v} \right). 
}
Intuitively, this pmf has a probability mass of $\alpha$  near $k \approx (1-\theta)2^v$, and no other probability mass anywhere.
% More precisely, we establish the following lemma.
This is made precise in the following lemma.
\begin{lemma} \label{lem:pmf}
If 
$\K = \{ k \big| \ \  |k \, 2^{-v} - (1-\theta)| \leq 2^{-(v-1)}\}$, 
then
% For any $j \in [1:u]$, 
% \aln{
% \Pr \left( (1-\beta) - 2^{-(v-1)} \leq [m_{1,j}/n]_v - [m_{2,j}/n]_v \leq (1-\beta) + 2^{-(v-1)} \right). 
% }
\al{
\sum_{k \in \K} p_j(k) \geq \alpha - \ep_n,
\label{eq:lemeq1}
}
where $\lim_{n\to \infty} \ep_n = 0$.
Moreover,
\al{
\max \{ p_j(k) : k \notin \K \} \leq 
2^{-(v-1)}. \label{eq:lemeq2}
% \frac{1}{\b2^}.
}
\end{lemma}
Given the lemma, we can bound the expected distortion as follows.
First, notice that the set $\K$ from Lemma~\ref{lem:pmf} has cardinality at most $5$.
Hence, for $n$ large enough, there is at least one value of $k \in \K$ with $p_j(k) \geq \alpha/6$.

% Notice that, while the random variables $[ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v$, $1 \leq j \leq u$, are not technically independent, as $n \to \infty$, they are essentially independent.
% This is because, given the location $m_{i,j}$ of the lexicographically first suffix based on one 
Notice that, if we view each of the $u$ masks $Z$ as drawn independently and uniformly at random from $\{0,1\}^n$, $(m_{1,j},m_{2,j})$ is independent of $(m_{1,\ell},m_{2,\ell})$ for $j \ne \ell$.
Hence, the random variables $[ m_{1,j}/n ]_v - [ m_{2,j}/n ]_v$, for $1 \leq j \leq u$, are independent (and identically distributed).
Notice that there are at most $u$ values in $\A$.
Using the union bound, Hoeffding's inequality, and (\ref{eq:lemeq2}),  the probability that there is a value $k2^{-v}$ for $k \notin \K$ that appears more than $\alpha_0 u$ times in $\A$ is at most
\al{
u \exp \left[ -2 u ( \alpha_0 - 2^{-(v-1)})^2 \right],
\label{eq:alpha0u}
}
for any $\delta > 0$,
as long as $\alpha_0 > 2^{-(v-1)}$ \iscomment{set $\alpha_0$}.

Now we analyze the resulting distortion by considering two separate cases, depending on the value of $\alpha$.
If $\alpha > 6 \alpha_0$, then the probability that, for no $k \in \K$, $k2^{-v}$ appears at least $\alpha_0 u$ times is at most
\aln{
\exp \left( -2 u (\alpha/5 - \alpha_0)^2 \right)
\leq \exp \left( -2 u (\alpha_0/5)^2 \right).
}
Notice that, as long as $\alpha_0 - 2^{-(v-1)} > \alpha_0/5
\Leftrightarrow \alpha_0 > \tfrac54 2^{-(v-1)}$, 
% \Rightarrow \alpha_0 > 2^{-(v-1)}$, 
% By setting $\delta = \alpha/12$, we conclude that, if 
% $\alpha/12 > 2^{-(v-1)}$, 
the probability that the resulting estimator is $\hat \theta = k \, 2^{-v}$ for some $k \notin \K$ is at most 
\al{
(u+1) \exp \left[ -2 u ( \alpha_0/5)^2 \right].
}
Therefore, when $\alpha > 6 \alpha_0$, the distortion satisfies
\al{
E & [(\theta-\hat \theta)^2| \alpha ]  \nonumber \\
& \leq \alpha 2^{-2(v-1)} 
+ (1-\alpha) (u+1) e^{-2u(\alpha_0/5)^2}.
% \nonumber \\
% &  \leq 2^{-2(v-1)} + (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)} )^2},
% \\
% &  \leq 25 \cdot 2^{-(v-1)} + (u+1) e^{-2u(\alpha/24)^2}. 
\label{eq:multipleloc2-case1}
}
Now we consider the second case, when $\alpha < 6 \alpha_0$.
In this case, $\theta = \frac{2\alpha}{1+\alpha} < 12 \alpha_0$.
Notice that, if there is no value $k2^{-v}$ for $k \notin \K$ that appears more than $\alpha_0 u$ times in $\A$, then we either have $\hat \theta = 0$ or $\hat \theta = k 2^{-v}$ for some $k \in \K$.
Using (\ref{eq:alpha0u} again, we conclude that, when $\alpha < 6 \alpha_0$, 
the distortion satisfies
\al{
E & [(\theta-\hat \theta)^2| \alpha ]  
% \nonumber \\
% & 
\leq 
\max( (12\alpha_0)^2, 2^{-2(v-1)} )
+ u e^{-2u(\alpha_0/5)^2}.
% & \leq \alpha 2^{-2(v-1)} 
% + (1-\alpha) (u+1) e^{-2u(\alpha_0/5)^2}.
\label{eq:multipleloc2-case2}
}
If we set $\alpha_0 = \tfrac{1}{12} 2^{-(v-1)}$,
we obtain a general bound 
\al{
E & [(\theta-\hat \theta)^2| \alpha ]  \nonumber \\
& \leq 2^{-2(v-1)} 
+ (u+1) e^{-2u(2^{-(v-1)}/60)^2}.
\label{eq:multipleloc2-combined}
}



it still holds that the probability that there is a value  is at most (\ref{eq:alpha0u}).
Hence, 



If $\alpha \leq \alpha_0{\bf /2}$, then the probability that the estimator outputs some






% Thus, we can use Hoeffding's inequality to establish that 



% Notice that there are at most $u$ values in $\A$.
% Using the union bound, Hoeffding's inequality, and (\ref{eq:lemeq2}),  the probability that there is a value $k2^{-v}$ for $k \notin \K$ that appears more than $(\alpha/6 - \delta)u$ times in $\A$ is at most
% \al{
% u \exp \left[ -2 u ( \alpha/6 - \delta - 2^{-(v-1)})^2 \right],
% }
% for any $\delta > 0$,
% as long as $\alpha/6 - \delta > 2^{-(v-1)}$.
% IS: Moving this up:
% Moreover, the probability that, for no $k \in \K$, $k2^{-v}$ appears at least $(\alpha/6-\delta)u$ times is at most
% $\exp \left( -2 u \delta ^2 \right)$.
By setting $\delta = \alpha/12$, we conclude that, if 
$\alpha/12 > 2^{-(v-1)}$, the probability that the resulting estimator is $\hat \theta = k \, 2^{-v}$ for some $k \notin \K$ is at most 
\al{
(u+1) \exp \left[ -2 u ( \alpha/12 - 2^{-(v-1)})^2 \right].
}
We conclude that the expected distortion can bounded as 
\al{
E & [(\theta-\hat \theta)^2| \alpha ]  \nonumber \\
& \leq \alpha 2^{-2(v-1)} 
+ (1-\alpha) (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)} )^2} \nonumber \\
&  \leq 2^{-2(v-1)} + (u+1) e^{-2u(\alpha/12 - 2^{-(v-1)} )^2},
% \\
% &  \leq 25 \cdot 2^{-(v-1)} + (u+1) e^{-2u(\alpha/24)^2}. 
\label{eq:multipleloc2}
}
as long as $\alpha/12 \leq 2^{-(v-1)}$.
Since $\alpha$ is uniformly distributed in $(0,1)$,
$\Pr(\alpha/24 \leq 2^{-(v-1)}) = 24 \cdot 2^{-(v-1)}$, and by averaging (\ref{eq:multipleloc2}) over $\alpha$, we obtain
\aln{
E [(\theta-\hat \theta)^2 ] &  \leq  24 \cdot 2^{-(v-1)} + 2^{-2(v-1)}  \nonumber \\
& \quad  + (u+1) E_\alpha \left[ e^{-2u(\alpha/12 - \alpha/24 )^2} \right] \\
&  \leq 25 \cdot 2^{-(v-1)} + (u+1) E_\alpha \left[ e^{-2u(\alpha/24)^2}\right] \\
& = 25 \cdot 2^{-(v-1)} + (u+1) \frac{\sqrt{\pi} (1-2Q(\sqrt{u} /12))}{2\sqrt{2 u}  /24}
% \label{eq:multipleloc2}
}
% \iscomment{It looks like this doesn't decay exponentially in $u$?}
% \iscomment{To get exponential decay, we need to assume that $\alpha$ is bounded away from zero. It makes sense since for $\alpha$ close to zero, the estimator is not good}


% \iscomment{what is a good way to bound that integral?}








